Analytic formulas for the rapid evaluation of the orbit response matrix and chromatic functions from lattice parameters in circular accelerators

Measurements and analysis of orbit response matrix have been providing for decades a formidable tool in the detection of linear lattice imperfections and their correction. Basically all storage-ring-based synchrotron light sources across the world make routinely use of this technique in their daily operation, reaching in some cases a correction of linear optics down to 1% beta beating and 0.1% coupling. During the design phase of a new storage ring it is also applied in simulations for the evaluation of magnetic and mechanical tolerances. However, this technique is known for its intrinsic slowness compared to other methods based on turn-by-turn beam position data, both in the measurement and in the data analysis. In this paper analytic formulas are derived and discussed that shall greatly speed up this second part. The mathematical formalism based on the Lie algebra and the resonance driving terms is extended to the off-momentum regime and explicit analytic formulas for the evaluation of chromatic functions from lattice parameters are also derived. The robustness of these formulas, which are linear in the magnet strengths, is tested with different lattice configurations.

==> app3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Corrections for the variation of the lattice parameters
                 across magnets}
\label{app:3}
All equations derived in the previous appendices have been 
derived assuming constant values for the beta and 
dispersion functions ($\beta_m$ and $D_m$) across a 
generic magnet $m$, usually computed at its center. 
The phase advance $\Delta\phi_{mj}$ between 
the magnet and a generic location $j$ refers to 
its center too. This approximation may not be sufficiently 
accurate in general and in particular for lattices 
comprising combined-function 
magnets, along which the beta function varies 
considerably. It is then of interest to evaluate 
corrections to the final equations of 
Secs.~\ref{ORM-Formulas}-\ref{CHROM-Formulas}
accounting for that variation. In doing so, another 
approximation is implicitly performed: Magnets  
are assumed to be hard-edged, i.e. their effective 
strengths are constant along the magnets and fall 
immediately to zero at their (magnetic) ends. The 
edge focusing at the dipole ends is also neglected. 
In Eq.~\eqref{eq:Nmatrix1} steerers $w$ are also assumed 
to be thin elements. In ring-based light sources orbit 
correctors are usually obtained from trim coils installed 
on sextupole magnets, and this approximation is usually 
rather robust. On the other hand, in rings making use 
of trim coils on bending magnets the variation of the 
lattice parameters across them may be no longer neglected. 
At the end of this section an approximate generalization 
accounting for thick steerers and sextupoles is 
eventually presented. 

In order to account for variation of the lattice 
parameters across the magnets, all terms dependent 
on $m$ in the formulas of 
Secs.~\ref{ORM-Formulas}-\ref{CHROM-Formulas} need 
to be replaced by their integral forms
\begin{eqnarray}
\beta_{m}\quad &\longrightarrow&\quad I_{\beta,m}=\frac{1}{L_m}
 \int_0^{L_m}{\beta(s)_{\ }ds}\ ,\qquad\label{eq:Ib1}\\
\beta_{m}\sin{(2\tau_{mj})}\quad &\longrightarrow&\quad\label{eq:IS1}
I_{S,mj}=\frac{1}{L_m}
 \int_0^{L_m}{\beta(s)\sin{(2\tau_{sj})}_{\ }ds}=\frac{1}{L_m}
 \int_0^{L_m}{\beta(s)\sin{(2\tau_{s_{m}j}- 2\Delta\phi_{s})}_{\ }ds}\ ,\qquad\\
\beta_{m}\cos{(2\tau_{mj})}\quad &\longrightarrow&\quad\label{eq:IC1}
I_{C,mj}=\frac{1}{L_m}
 \int_0^{L_m}{\beta(s)\cos{(2\tau_{sj})}_{\ }ds}=\frac{1}{L_m}
 \int_0^{L_m}{\beta(s)\cos{(2\tau_{s_{m}j}- 2\Delta\phi_{s})}_{\ }ds}\ ,\qquad\\
\sqrt{\beta_{m}}\sin{(\tau_{mj})}\quad &\longrightarrow&\quad\label{eq:JS1}
J_{C,mj}=\frac{1}{L_m}\int_0^{L_m}
{\hskip-2mm\sqrt{\beta(s)}\sin{(\tau_{sj})}_{\ }ds}=\frac{1}{L_m}
\int_0^{L_m}{\hskip-2mm\sqrt{\beta(s)}\sin{(\tau_{s_{m}j}-\Delta\phi_s)}_{\ }ds}\ ,\qquad\\
\sqrt{\beta_{m}}\cos{(\tau_{mj})}\quad &\longrightarrow&\quad\label{eq:JC1}
J_{C,mj}=\frac{1}{L_m}\int_0^{L_m}
{\hskip-2mm\sqrt{\beta(s)}\cos{(\tau_{sj})}_{\ }ds}=\frac{1}{L_m}
\int_0^{L_m}{\hskip-2mm\sqrt{\beta(s)}\cos{(\tau_{s_{m}j}-\Delta\phi_s)}_{\ }ds}\ ,\qquad\\
\sqrt{\beta_{m,x}}D_{m,y}\cos{(\tau_{x,mj})}\quad &\longrightarrow&\quad\label{eq:JCDy}
J_{C,mj}^{(D_y)}=\frac{1}{L_m}\int_0^{L_m}
{\sqrt{\beta_x(s)}D_y(s)\cos{(\tau_{x,s_{m}j}-\Delta\phi_{x,s})}_{\ }ds}\ ,\qquad\\
\sqrt{\beta_{m,y}}D_{m,x}\cos{(\tau_{y,mj})}\quad &\longrightarrow&\quad\label{eq:JCDx}
J_{C,mj}^{(D_x)}=\frac{1}{L_m}\int_0^{L_m}
{\sqrt{\beta_y(s)}D_x(s)\cos{(\tau_{y,s_{m}j}-\Delta\phi_{y,s})}_{\ }ds}\ ,\qquad
\end{eqnarray}
where $L_m$ denotes the length of the magnet $m$, 
$s_{m}$ represents the position along the ring of its entrance 
whereas $\Delta\phi_{s}$ is the phase advance along the magnet. 

%%%%%--------------------------------------------------------------------------
\subsection{$I_{\beta,m},\ I_{S,mj}$ and $I_{C,mj}$ for quadrupoles}
The above integrals enter in Eq.~\eqref{eq:Nmatrix1} to 
account for the variation of the C-S parameters across 
quadrupoles in the evaluation of the diagonal ORM blocks. 
They can be solved by making use of the two 
representations of the transfer matrix along the magnet, 
i.e. from it entrance $s_{m}=0$ and the generic position $s$
\begin{eqnarray}
\mathbf{A_m}(s)=\left\{
\begin{aligned}
\left(\begin{array}{c c}
\cos{(\sqrt{k_m}s)}            & \frac{1}{\sqrt{k_m}}\sin{(\sqrt{k_m}s)} \\
-\sqrt{k_m}\sin{(\sqrt{k_m}s)} & \cos{(\sqrt{k_m}s)}
\end{array} \right) \qquad&\hbox{focusing plane}\\
\left(\begin{array}{c c}
\cosh{(\sqrt{|k_m|}s)}           & \frac{1}{\sqrt{|k_m|}}\sinh{(\sqrt{|k_m|}s)} \\
\sqrt{|k_m|}\sinh{(\sqrt{|k_m|}s)} & \cosh{(\sqrt{|k_m|}s)}
\end{array} \right) \qquad&\hbox{defocusing plane}\
\end{aligned}\right. \quad ,\label{eq:Adef1}\\
\mathbf{C_m}(s)=
\left(\begin{array}{c c}
\sqrt{\frac{\beta(s)}{\beta_{m0}}}\left(\cos{\Delta\phi_s}+
\alpha_{m0}\sin{\Delta\phi_s}\right) & 
\sqrt{\beta(s)\beta_{m0}}\sin{\Delta\phi_s} \\
\frac{\alpha_{m0}-\alpha(s)}{\sqrt{\beta(s)\beta_{m0}}}\cos{\Delta\phi_s}
-\frac{1-\alpha_{m0}\alpha(s)}{\sqrt{\beta(s)\beta_{m0}}}\sin{\Delta\phi_s} &
\sqrt{\frac{\beta_{m0}}{\beta(s)}}\left(\cos{\Delta\phi_s}+
\alpha(s)\sin{\Delta\phi_s}\right)
\end{array} \right)\quad ,\label{eq:Cdef1}
\end{eqnarray}
where $k_m$ represents the model non-integrated quadrupole 
strength, whereas $\beta_{m0}$ and $\alpha_{m0}$ are 
the C-S parameters at the quadrupole entrance, both computed 
from the ideal model. By imposing 
that $A_{m,11}=C_{m,11}$ and $A_{m,12}=C_{m,12}$ we obtain
\begin{eqnarray}\left\{
\begin{aligned}
\sqrt{\beta(s)}\sin{\Delta\phi_s}&=\frac{1}{\sqrt{|k_m|\beta_{m0}}}
\left(\begin{array}{c}\sin{(\sqrt{k_m}s)} \\ \sinh{(\sqrt{|k_m|}s)}
\end{array}\right) \\
\sqrt{\beta(s)}\cos{\Delta\phi_s}&=\sqrt{\beta_{m0}}
\left(\begin{array}{c}\cos{(\sqrt{k_m}s)} \\ \cosh{(\sqrt{|k_m|}s)}
\end{array}\right)
-\frac{\alpha_{m0}}{\sqrt{|k_m|\beta_{m0}}}
\left(\begin{array}{c}\sin{(\sqrt{k_m}s)} \\ \sinh{(\sqrt{|k_m|}s)}
\end{array}\right)
\end{aligned}\right. \quad ,\label{eq:ACmatrix}
\end{eqnarray}
where the upper and lower terms refer to the focusing and 
defocusing planes, respectively. By summing the square of 
the above equations the following expression for the beta 
function along the quadrupole is obtained
\begin{eqnarray}
\beta(s)=\frac{\gamma_{m0}}{|k_m|}\left(\begin{array}{c}
         \sin^2{(\sqrt{k_m}s)} \\ \sinh^2{(\sqrt{|k_m|}s)}\end{array}\right)
        +\beta_{m0}\left(\begin{array}{c}
         \cos^2{(\sqrt{k_m}s)} \\ \cosh^2{(\sqrt{|k_m|}s)}\end{array}\right)
        -\frac{\alpha_{m0}}{\sqrt{|k_m|}}\left(\begin{array}{c}
         \sin{(2\sqrt{k_m}s)} \\ \sinh{(2\sqrt{|k_m|}s)}\end{array}\right)
\quad ,\label{eq:beta_quad}
\end{eqnarray}
where $\gamma_{m0}=(1+\alpha_{m0}^2)/\beta_{m0}$ is the 
third C-S parameter. After inserting the above expression 
in the integral of Eq.~\eqref{eq:Ib1} and applying the 
following relations, 
\begin{eqnarray} \label{eq:integr1}
\begin{aligned}
\int_0^{L_m}{\sin^2{(\sqrt{k_m}s)} ds}=\frac{L_m}{2}-
       \frac{\sin{(2\sqrt{k_m}L_m)}}{4\sqrt{k_m}}\quad&,\quad
\int_0^{L_m}{\sinh^2{(\sqrt{|k_m|}s)} ds}=-\frac{L_m}{2}+
       \frac{\sinh{(2\sqrt{|k_m|}L_m)}}{4\sqrt{|k_m|}}\quad ,  \\
\int_0^{L_m}{\cos^2{(\sqrt{k_m}s)} ds}=\frac{L_m}{2}+
       \frac{\sin{(2\sqrt{k_m}L_m)}}{4\sqrt{k_m}}\quad&,\quad
\int_0^{L_m}{\cosh^2{(\sqrt{|k_m|}s)} ds}=\ \frac{L_m}{2}+
       \frac{\sinh{(2\sqrt{|k_m|}L_m)}}{4\sqrt{|k_m|}}\quad ,\\
\int_0^{L_m}{\sin{(2\sqrt{k_m}s)} ds}=\frac{1}{2\sqrt{k_m}}-
       \frac{\cos{(2\sqrt{k_m}L_m)}}{2\sqrt{k_m}}\quad&,\quad
\int_0^{L_m}{\sinh{(2\sqrt{|k_m|}s)} ds}=-\frac{1}{2\sqrt{|k_m|}}+
       \frac{\cosh{(2\sqrt{|k_m|}L_m)}}{2\sqrt{|k_m|}}\quad ,
\end{aligned}
\end{eqnarray}
the following expression for the correction term 
$I_{\beta,m}$ is obtained
\begin{eqnarray}
I_{\beta,m}=\left\{
\begin{aligned}
&\frac{1}{2}\left[\beta_{m0}+\frac{\gamma_{m0}}{k_m}\right]
+\hskip 1mm \frac{\sin{(2\sqrt{k_m}L_m)}}{4\sqrt{k_m}L_m}\hskip 1mm
      \left[\beta_{m0}-\frac{\gamma_{m0}}{k_m}\right]
+\hskip 1mm \frac{\alpha_{m0}}{2k_mL_m}\hskip 1mm
       \left[\cos{(2\sqrt{k_m}L_m)}-1\right] 
\hskip8mm \hbox{focusing plane}\\
&\frac{1}{2}\left[\beta_{m0}-\frac{\gamma_{m0}}{|k_m|}\right]
+\frac{\sinh{(2\sqrt{|k_m|}L_m)}}{4\sqrt{|k_m|}L_m}
      \left[\beta_{m0}+\frac{\gamma_{m0}}{|k_m|}\right]
-\frac{\alpha_{m0}}{2|k_m|L_m}
       \left[\cosh{(2\sqrt{|k_m|}L_m)}-1\right]
\ \hbox{defocusing plane}
\end{aligned}\right. .\nonumber
\end{eqnarray}
The two cases, focusing ($k_m>0$) and defocusing ($k_m<0$) quadrupoles,
can be actually described by a single formula
\begin{eqnarray}\displaystyle
I_{\beta,m}=\frac{1}{2}\left[\beta_{m0}+\frac{\gamma_{m0}}{k_m}\right]
+\hskip 1mm \frac{\sin{(2\sqrt{k_m}L_m)}}{4\sqrt{k_m}L_m}\hskip 1mm
      \left[\beta_{m0}-\frac{\gamma_{m0}}{k_m}\right]
+\hskip 1mm \frac{\alpha_{m0}}{2k_mL_m}\hskip 1mm
       \left[\cos{(2\sqrt{k_m}L_m)}-1\right] \ , \label{eq:Ib2}
\end{eqnarray}
since for $k_m<0$ $\sin{(2\sqrt{k_m}L_m)}/\sqrt{k_m}=
\sinh{(2\sqrt{|k_m|}L_m)}/\sqrt{|k_m|}$ and $\cos{(2\sqrt{k_m}L_m)}=
\cosh{(2\sqrt{|k_m|}L_m)}$. 
The trigonometric integrals of Eqs.~\eqref{eq:IS1}-\eqref{eq:IC1}
can be rewritten as
\begin{eqnarray}\label{eq:IS2}
\begin{aligned}
I_{S,mj}&=\sin{(2\tau_{s_{m}j})}I_{C,m}-\cos{(2\tau_{s_{m}j})}I_{S,m}
\quad ,\quad I_{C,m}=\frac{1}{L_m}
 \int_0^{L_m}{\beta(s)\cos{(2\Delta\phi_{s})}_{\ }ds}\ ,\\
I_{C,mj}&=\cos{(2\tau_{s_{m}j})}I_{C,m}+\sin{(2\tau_{s_{m}j})}I_{S,m}
\quad ,\quad I_{S,m}=\frac{1}{L_m}
 \int_0^{L_m}{\beta(s)\sin{(2\Delta\phi_{s})}_{\ }ds}\ .
\end{aligned} 
\end{eqnarray}
In the above expressions $\tau_{s_{m}j}=\Delta\phi_{s_{m}j}-\pi Q$ 
represents the shifted phase advance between the 
generic location $j$ and the entrance of the 
magnet $m$ ($s_{m}$), whereas the integrals $I_{C,m}$ 
and $I_{S,m}$ depend on the magnet $m$ only. By making use 
of the relation $\cos{(2\Delta\phi_{s})}=1-2\sin^2{\Delta\phi_{s}}$, 
replacing $\beta(s)\sin^2{\Delta\phi_{s}}$ with the first 
expression in Eq.~\eqref{eq:ACmatrix}, and applying the 
integrals of Eq.~\eqref{eq:integr1}, the first integral reads
\begin{eqnarray}\label{eq:IC2}
  I_{C,m}=I_{\beta,m}-
  \frac{1}{k_m\beta_{m0}}\left[\hskip1mm 1-
        \frac{\sin{(2\sqrt{k_m}L_m)}}{2\sqrt{k_m}L_m}\right] 
         \quad ,
\end{eqnarray}
which is valid for both focusing and defocusing quadrupoles,
as for Eq.~\eqref{eq:Ib2} ($\sin{(2\sqrt{k_m}L_m)}/\sqrt{k_m}=
\sinh{(2\sqrt{|k_m|}L_m)}/\sqrt{|k_m|}$ for $k_m<0$).
The second integral can be computed by replacing 
$\beta(s)\sin{(2\Delta\phi_{s})}=2(\sqrt{\beta(s)}\sin{\Delta\phi_{s}})
(\sqrt{\beta(s)}\cos{\Delta\phi_{s}})$, by substituting the 
terms in the parenthesis with the expressions of 
Eq.~\eqref{eq:ACmatrix}, and by making use of the 
integrals of Eq.~\eqref{eq:integr1}. The result is 
\begin{eqnarray}\label{eq:IS3}
I_{S,m}=\frac{1}{k_mL_m}\left[\hskip2mm\frac{1}{2}\left(1-\cos{(2\sqrt{k_m}L_m)}
       \right)+\frac{\alpha_{m0}}{\beta_{m0}}\left(
       \frac{\sin{(2\sqrt{k_m}L_m)}}{2\sqrt{k_m}}-L_m\right)\right]   \ .\qquad
\end{eqnarray} 
 

%%%%%--------------------------------------------------------------------------
\subsection{$J_{S,mj}$ and $J_{C,mj}$ for sector dipoles}
$J_{C,mj}$  enters in Eq.~\eqref{eq:Text_Disp1} to account for 
the evolution of the C-S parameters across a dipole magnet in the 
evaluation of the dispersion function. $J_{S,mj}$ is evaluated 
for completeness.

The transfer matrix $\mathbf{A_m}$ for a sector dipole reads
\begin{eqnarray}
\mathbf{A_m}(s)=\left(\begin{array}{c c}
\cos{(K_{m,0})}                             & \rho\sin{(K_{m,0})} \\
\displaystyle-\frac{1}{\rho}\sin{(K_{m,0})} & \cos{(K_{m,0})}
\end{array} \right) \quad = \quad
\left(\begin{array}{c c}\displaystyle
\cos{(K_{m,0})}  & \displaystyle\frac{s}{K_{m,0}}\sin{(K_{m,0})} \\
\displaystyle-\frac{K_{m,0}}{s}\sin{(K_{m,0})} & \cos{(K_{m,0})}
\end{array} \right) \qquad .\label{eq:Adef2}
\end{eqnarray}
As in the previous case, by imposing that 
$A_{m,11}=C_{m,11}$ and $A_{m,12}=C_{m,12}$, 
the elements of the $\mathbf{C_m}$ matrix 
being the same of Eq.~\eqref{eq:Cdef1}, we obtain
\begin{eqnarray}\left\{
\begin{aligned}
\sqrt{\beta(s)}\sin{\Delta\phi_s}&=
             \frac{\sin{K_{m,0}}}{K_{m,0}\sqrt{\beta_{m0}}}\ s\\
\sqrt{\beta(s)}\cos{\Delta\phi_s}&=\sqrt{\beta_{m0}}\cos{K_{m,0}}-
             \frac{\alpha_{m0}\sin{K_{m,0}}}{K_{m,0}\sqrt{\beta_{m0}}}\ s
\end{aligned}\right. \quad .\label{eq:ACmatrix2}
\end{eqnarray}
By integrating the above expressions across the magnet yields
\begin{eqnarray}
\begin{aligned}\label{eq:JCmj0}
T_{S,m}&=\frac{1}{L_m}\int_0^{L_m}{\sqrt{\beta(s)}\sin{\Delta\phi_s}\ ds}=
             \frac{L_m\sin{K_{m,0}}}{2K_{m,0}\sqrt{\beta_{m0}}}\quad ,\\
T_{C,m}&=\frac{1}{L_m}\int_0^{L_m}{\sqrt{\beta(s)}\cos{\Delta\phi_s}\ ds}=
\sqrt{\beta_{m0}}\cos{K_{m,0}}-
             \frac{\alpha_{m0}L_m\sin{K_{m,0}}}{2K_{m,0}\sqrt{\beta_{m0}}}\quad ,
\end{aligned} 
\end{eqnarray}
$J_{S,mj}$ and $J_{C,mj}$ for sector dipoles can be eventually 
written and computed as 
\begin{eqnarray}\label{eq:JCmj1}
\begin{aligned}
J_{S,mj}&=\sin{(\tau_{s_{m}j})}T_{C,m}-\cos{(\tau_{s_{m}j})}T_{S,m}\quad , \\
J_{C,mj}&=\cos{(\tau_{s_{m}j})}T_{C,m}+\sin{(\tau_{s_{m}j})}T_{S,m}\quad ,
\end{aligned}
\end{eqnarray}
where, as usual, $\tau_{s_{m}j}$ is the shifted phase 
advance between the entrance of the magnet $m$ and 
the observation point $j$.


%%%%%--------------------------------------------------------------------------
\subsection{$J_{S,mj}$ and $J_{C,mj}$ for quadrupoles and combined-function dipoles}
$J_{C,mj}$  enters in Eq.~\eqref{eq:Text_Disp1} to account for 
the evolution of the C-S parameters across a combined-function 
dipole magnet in the evaluation of the dispersion function. 
Both $J_{S,mj}$ and $J_{C,mj}$ are also needed in the evaluation 
of the integrals of Eq.~\eqref{eq:Smatrix1-thick} for the 
computation of the off-diagonal ORM block. 

As far as the betatron motion, the transfer matrix of a 
combined-function dipole is the one of simple quadrupole 
(the same is not true for dispersive terms). 
The integration of both sides and equations of 
Eq.~\eqref{eq:ACmatrix} reads
\begin{eqnarray}
\begin{aligned}
G_{S,m}&=\frac{1}{L_m}\int_0^{L_m}{\sqrt{\beta(s)}\sin{\Delta\phi_s}\ ds}=
         \frac{1}{L_m\sqrt{k_m\beta_{m0}}}\int_0^{L_m}{\sin{(\sqrt{k_m}s)}
         \ ds}   \quad ,\\
G_{C,m}&=\frac{1}{L_m}\int_0^{L_m}{\sqrt{\beta(s)}\cos{\Delta\phi_s}\ ds}=
         \frac{\sqrt{\beta_{m0}}}{L_m}\int_0^{L_m}{\cos{(\sqrt{k_m}s)}\ ds}
         -\frac{\alpha_{m0}}{L_m\sqrt{k_m\beta_{m0}}}
          \int_0^{L_m}{\sin{(\sqrt{k_m}s)}\ ds} \quad .
\end{aligned} 
\end{eqnarray}
Once again the above expressions holds both for focusing and 
defocusing quadrupoles, since for $k_m<0$ $\sin{(2\sqrt{k_m}L_m)}/\sqrt{k_m}=
\sinh{(2\sqrt{|k_m|}L_m)}/\sqrt{|k_m|}$ and $\cos{(2\sqrt{k_m}L_m)}=
\cosh{(2\sqrt{|k_m|}L_m)}$. The result is 
\begin{eqnarray}
\begin{aligned}\label{eq:JCmj2}
G_{S,m}&=\frac{1}{L_m k_m\sqrt{\beta_{m0}}}\left[1-\cos{(\sqrt{k_m}L_m)}
         \right]\quad ,\\
G_{C,m}&=\frac{\sqrt{\beta_{m0}}}{L_m\sqrt{k_m}}\sin{(\sqrt{k_m}L_m)}
         -\frac{\alpha_{m0}}{L_m k_m\sqrt{\beta_{m0}}}
          \left[1-\cos{(\sqrt{k_m}L_m)}\right] \quad .
\end{aligned} 
\end{eqnarray}
$J_{S,mj}$ and $J_{C,mj}$ for quadrupoles and combined-function 
magnets can be eventually written and computed as 
\begin{eqnarray}\label{eq:JCmj3}
\begin{aligned}
J_{S,mj}&=\sin{(\tau_{s_{m}j})}G_{C,m}-\cos{(\tau_{s_{m}j})}G_{S,m}\quad , \\
J_{C,mj}&=\cos{(\tau_{s_{m}j})}G_{C,m}+\sin{(\tau_{s_{m}j})}G_{S,m}\quad ,
\end{aligned}
\end{eqnarray}
where $\tau_{s_{m}j}$ is again the shifted phase 
advance between the entrance of the magnet $m$ and 
the observation point $j$.

%%%%%--------------------------------------------------------------------------
\subsection{$J_{C,mj}^{(D_y)}$  and $J_{C,mj}^{(D_x)}$  for quadrupoles}
These integrals can be used  in the evaluation of 
the dispersion function from Eq.~\eqref{eq:Text_Disp1} 
to account for the evolution of the C-S parameters and 
dispersion across a skew quadrupole magnet. 

Differently from the integrals $I$ and $J$ discussed in 
the previous sections, the $J^{(D)}$ integrals 
contain the dispersion function (in the orthogonal 
plane), whose propagation along the quadrupole 
needs to be evaluated separately. The following 
expression applies for a generic combined-function 
magnet
\begin{eqnarray}\label{eq:Transport1}
\left(\begin{array}{c} D(s) \\ D'(s) \\ 1\end{array}\right)=
\left(\begin{array}{c c}\mathbf{A_m}(s)&\vec{d}\\ 0 & 1\end{array}\right)
\left(\begin{array}{c} D_{m,0} \\ D'_{m,0} \\ 1\end{array}\right)
\quad ,
\end{eqnarray}
where $D_{m,0}$ and $D'_{m,0}$ are the dispersion 
and its derivative at the entrance of the magnet, 
$\mathbf{A_m}$ is the betatron matrix of 
Eq.~\eqref{eq:Adef2} for a pure sector dipole, 
of Eq.~\eqref{eq:Adef1} otherwise. For 
quadrupoles $\vec{d}=(0 \ 0)^T$ and dispersion is 
propagated according to 
\begin{eqnarray}
D(s)&=D_{m0}\left(\begin{array}{c}
             \cos{(\sqrt{k_m}s)} \\ \cosh{(\sqrt{|k_m|}s)}
             \end{array}\right) 
     +\frac{D'_{m0}}{\sqrt{|k_m|}}\left(\begin{array}{c}
             \sin{(\sqrt{k_m}s)} \\ \sinh{(\sqrt{|k_m|}s)}
             \end{array}\right)\ ,
\end{eqnarray}
where, once again, the upper and lower terms 
refer to the focusing and defocusing planes, 
respectively. By merging the above expression 
with the ones in Eq.~\eqref{eq:ACmatrix}, 
the following relations are obtained
\begin{eqnarray}\label{eq:T1}
\begin{aligned}
T_{S,x,m}&=\frac{1}{L_m}\int_0^{L_m}{\hskip -2mm\sqrt{\beta_x(s)}D_y(s)
            \sin{\Delta\phi_{x,s}}\ ds}= 
            \frac{D_{y,m0}}{L_m\sqrt{|k_m|\beta_{x,m0}}}
            \int_0^{L_m}\hskip -1mm\left(\begin{array}{l}
             \cosh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)} \\ 
             \sinh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)}
             \end{array}\right) ds\\ &\hskip3mm
          +\frac{D'_{y,m0}}{|k_m|L_m\sqrt{\beta_{x,m0}}}
           \int_0^{L_m}\hskip -3mm
           \sin{(\sqrt{|k_m|}s)}\sinh{(\sqrt{|k_m|}s)} ds\quad ,\\
T_{C,x,m}&=\frac{1}{L_m}\int_0^{L_m}{\hskip -2mm\sqrt{\beta_x(s)}D_y(s)
           \cos{\Delta\phi_{x,s}}\ ds}= 
           \frac{\sqrt{\beta_{x,m0}}D_{y,m0}}{L_m}\int_0^{L_m}\hskip -3mm
           \cosh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)}\ ds\\&\hskip3mm
          -\frac{\alpha_{x,m0}D'_{y,m0}}{L_m|k_m|\sqrt{\beta_{x,m0}}}
           \int_0^{L_m}\hskip -3mm
           \sinh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)}\ ds
          -\frac{\alpha_{x,m0}D_{y,m0}}{L_m\sqrt{|k_m|\beta_{x,m0}}}
           \int_0^{L_m}\hskip -1mm\left(\begin{array}{c}
             \cosh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)} \\ 
             \sinh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)}
             \end{array}\right) ds\\&\hskip3mm
          +\frac{\sqrt{\beta_{x,m0}}D'_{y,m0}}{L_m\sqrt{|k_m|}}
           \int_0^{L_m}\hskip -1mm\left(\begin{array}{c}
             \sinh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)} \\
             \cosh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)}
             \end{array}\right) ds \quad ,\\
T_{S,y,m}&=\frac{1}{L_m}\int_0^{L_m}{\hskip -2mm\sqrt{\beta_y(s)}D_x(s)
            \sin{\Delta\phi_{y,s}}\ ds}= 
            \frac{D_{x,m0}}{L_m\sqrt{|k_m|\beta_{y,m0}}}
            \int_0^{L_m}\hskip -1mm\left(\begin{array}{l}
             \sinh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)} \\
             \cosh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)} 
             \end{array}\right) ds\\ &\hskip3mm
          +\frac{D'_{x,m0}}{|k_m|L_m\sqrt{\beta_{y,m0}}}
           \int_0^{L_m}\hskip -3mm
           \sin{(\sqrt{|k_m|}s)}\sinh{(\sqrt{|k_m|}s)} ds\quad ,\\
T_{C,y,m}&=\frac{1}{L_m}\int_0^{L_m}{\hskip -2mm\sqrt{\beta_y(s)}D_x(s)
            \cos{\Delta\phi_{y,s}}\ ds}=  
           \frac{\sqrt{\beta_{y,m0}}D_{x,m0}}{L_m}\int_0^{L_m}\hskip -3mm
           \cosh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)}\ ds\\&\hskip3mm
          -\frac{\alpha_{y,m0}D'_{x,m0}}{L_m|k_m|\sqrt{\beta_{y,m0}}}
           \int_0^{L_m}\hskip -3mm
           \sinh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)}\ ds
          -\frac{\alpha_{y,m0}D_{x,m0}}{L_m\sqrt{|k_m|\beta_{y,m0}}}
           \int_0^{L_m}\hskip -1mm\left(\begin{array}{c}
             \sinh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)} \\
             \cosh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)}  
             \end{array}\right) ds\\&\hskip3mm
          +\frac{\sqrt{\beta_{y,m0}}D'_{x,m0}}{L_m\sqrt{|k_m|}}
           \int_0^{L_m}\hskip -1mm\left(\begin{array}{c}
             \cosh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)} \\
             \sinh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)} 
             \end{array}\right) ds \quad .
\end{aligned}
\end{eqnarray}
Note that because of the presence of the dispersion 
of the orthogonal plane, the above integrals in the 
two planes have a different functional dependence on 
the quadrupole gradients $|k_m|$ (the integrals in the 
r.h.s. are swapped). The absolute value is introduced in 
the trigonometric functions too, in order account for the fact 
that when one plane is focusing, the other is defocusing though 
both the trigonometric and the hyperbolic functions will 
have always a positive argument: The use of the absolute 
value then avoids any conflict with the sign of $k_m$.

The four terms of Eq.~\eqref{eq:T1}
can be made explicit after computing and replacing 
four integrals
\begin{eqnarray}
\begin{aligned}
\int_0^{L_m}\hskip -3mm \cos{(\sqrt{|k_m|}s)}\cosh{(\sqrt{|k_m|}s)} ds &= 
  \frac{1}{2\sqrt{|k_m|}}\left[\sin{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}
           +\cos{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}\right]\ ,\\
\int_0^{L_m}\hskip -3mm \sin{(\sqrt{|k_m|}s)}\sinh{(\sqrt{|k_m|}s)} ds &= 
  \frac{1}{2\sqrt{|k_m|}}\left[\sin{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}
           -\cos{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}\right]\ ,\\
\int_0^{L_m}\hskip -3mm \cosh{(\sqrt{|k_m|}s)}\sin{(\sqrt{|k_m|}s)} ds &= 
  \frac{1}{2\sqrt{|k_m|}}\left[\sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
           -\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}+1\right]\ ,\\
\int_0^{L_m}\hskip -3mm \sinh{(\sqrt{|k_m|}s)}\cos{(\sqrt{|k_m|}s)} ds &=
  \frac{1}{2\sqrt{|k_m|}}\left[\sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
           +\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}-1\right]\ ,\\
\end{aligned}\nonumber 
\end{eqnarray}
resulting in 
\begin{eqnarray}\label{eq:T2}
\begin{aligned}
T_{S,x,m}&= \frac{D_{y,m0}}{2|k_m|L_m\sqrt{\beta_{x,m0}}}
            \left(\begin{array}{l}
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
           -\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}+1 \\ 
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
           +\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}-1
             \end{array}\right)\\ &\hskip3mm
          +\frac{D'_{y,m0}}{2|k_m|^{3/2}L_m\sqrt{\beta_{x,m0}}}
           \left[\sin{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}
           -\cos{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}\right]\quad ,\\
T_{C,x,m}&= 
           \frac{\sqrt{\beta_{x,m0}}D_{y,m0}}{2\sqrt{|k_m|}L_m}
           \left[\sin{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}
           +\cos{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}\right] \\&\hskip3mm
          -\frac{\alpha_{x,m0}D'_{y,m0}}{2|k_m|^{3/2}L_m\sqrt{\beta_{x,m0}}}
           \left[\sin{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}
                -\cos{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}\right]
           \\&\hskip3mm
-\frac{\alpha_{x,m0}D_{y,m0}}{2|k_m|L_m\sqrt{\beta_{x,m0}}}
           \left(\begin{array}{c}
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
            -\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}+1 \\
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
            +\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}-1
           \end{array}\right)
           \\&\hskip3mm
          +\frac{\sqrt{\beta_{x,m0}}D'_{y,m0}}{2|k_m|L_m}
           \left(\begin{array}{c}
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
            +\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}-1 \\
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
            -\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}+1
           \end{array}\right)
 \quad ,\\
T_{S,y,m}&=\frac{D_{x,m0}}{2|k_m|L_m\sqrt{\beta_{y,m0}}}
            \left(\begin{array}{l}
            \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
           +\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}-1 \\ 
            \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
           -\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}+1
             \end{array}\right)\\ &\hskip3mm
          +\frac{D'_{x,m0}}{2|k_m|^{3/2}L_m\sqrt{\beta_{y,m0}}}
           \left[\sin{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}
           -\cos{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}\right]\quad ,\\
T_{C,y,m}&= 
           \frac{\sqrt{\beta_{y,m0}}D_{x,m0}}{2\sqrt{|k_m|}L_m}
           \left[\sin{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}
           +\cos{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}\right] \\&\hskip3mm
          -\frac{\alpha_{y,m0}D'_{x,m0}}{2|k_m|^{3/2}L_m\sqrt{\beta_{y,m0}}}
           \left[\sin{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}
                -\cos{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}\right]
           \\&\hskip3mm
-\frac{\alpha_{y,m0}D_{x,m0}}{2|k_m|L_m\sqrt{\beta_{y,m0}}}
           \left(\begin{array}{c}
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
            +\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}-1 \\
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
            -\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}+1
           \end{array}\right)
           \\&\hskip3mm
          +\frac{\sqrt{\beta_{y,m0}}D'_{x,m0}}{2|k_m|L_m}
           \left(\begin{array}{c}
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
            -\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}+1 \\
             \sin{(\sqrt{|k_m|}L_m)}\sinh{(\sqrt{|k_m|}L_m)}
            +\cos{(\sqrt{|k_m|}L_m)}\cosh{(\sqrt{|k_m|}L_m)}-1
           \end{array}\right)
 \quad .
\end{aligned}
\end{eqnarray}
Once again, the upper and lower terms in the brackets 
refer to the focusing and defocusing planes, respectively.
By decomposing the cosine term within the integrals 
of Eqs.~\eqref{eq:JCDy}-\eqref{eq:JCDx}, $J_{C,mj}^{(D_y)}$ 
and $J_{C,mj}^{(D_x)}$ at the quadrupoles eventually 
read
\begin{eqnarray}\label{eq:JCDxy}
\begin{aligned}
J_{C,mj}^{(D_y)}&=\cos{(\tau_{x,s_mj})}T_{C,x,m}+
                  \sin{(\tau_{x,s_mj})}T_{S,x,m}\quad , \\
J_{C,mj}^{(D_x)}&=\cos{(\tau_{y,s_mj})}T_{C,y,m}+
                  \sin{(\tau_{y,s_mj})}T_{S,y,m}\quad ,
\end{aligned}
\end{eqnarray}
where the $T$ functions are those of Eq.~\eqref{eq:T2}, and 
$\tau_{s_mj}=\Delta\phi_{s_mj}-\pi Q$ 
represents the usual shifted phase advance between the 
generic location $j$ and the entrance of the 
magnet $m$ ($s_{m}$).

%%%%%--------------------------------------------------------------------------
\subsection{$J_{C,mj}^{(D_y)}$  and $J_{C,mj}^{(D_x)}$  for 
            combined-function magnets}
For the evaluation of the two integrals across 
combined-function magnets (i.e. with both dipole 
and quadrupole fields), the same calculations 
carried out in the previous section need to be 
repeated from Eq.~\eqref{eq:Transport1}, with a 
nonzero ($1\times2$) vector 
\begin{eqnarray}\label{eq:vectd-comb}
\vec{d}=
\left\{\begin{aligned}
&\left(\frac{1}{\rho k_m}(1-\cos{\sqrt{k_m}s})\quad 
      \frac{1}{\rho \sqrt{k_m}}\sin{\sqrt{k_m}s}\right)^T \\
&\left(\frac{1}{\rho|k_m|}(-1+\cosh{\sqrt{|k_m|}s})\quad 
      \frac{1}{\rho\sqrt{|k_m|}}\sinh{\sqrt{|k_m|}s}\right)^T
\end{aligned}\right. \qquad .
\end{eqnarray}
For the present ESRF storage ring, this calculation 
is not needed, though it shall be performed for 
machines such as the present ALBA and the new ESRF 
storage rings, both comprising defocusing 
combined-function dipoles, whose tilts may affect 
the dispersion function. 

%%%%%--------------------------------------------------------------------------
\subsection{Corrections for thick orbit deflectors and sextupoles}
\label{app:thicksteerers}
So far, integrals replacing constant terms have been 
derived for quadrupoles and combined-function magnets $m$, 
only, i.e. assuming thin steerers $w$ (along with thin 
BPMs $j$) for the ORM of Eq.~\eqref{eq:Nmatrix1} 
and thin sextupoles $m$ for the chromatic functions of 
Sec.~\ref{CHROM-Formulas}. In order to account for 
the variation of the C-S parameters across all magnets $m$ 
and deflectors $w$ in Eqs.~\eqref{eq:Nmatrix1},~\eqref{eq:Text_Chrom1}, 
\eqref{eq:Text_ChromBeat3},~\eqref{eq:Text-ChromPhAdx} 
and~\eqref{eq:Text-ChromPhAdy} the following terms 
need to be replaced
\begin{eqnarray}
\sqrt{\beta_{w}}\cos{(\tau_{wj})}\quad &\longrightarrow&\quad\label{eq:ICwj}
J_{C,wj}=\frac{1}{L_w}\int_0^{L_w}{\sqrt{\beta(s)}\cos{(\tau_{sj})}_{\ }ds}\ ,\\
\sqrt{\beta_{w}}\sin{(\tau_{wj})}\quad &\longrightarrow&\quad\label{eq:ISwj}
J_{C,wj}=\frac{1}{L_w}\int_0^{L_w}{\sqrt{\beta(s)}\sin{(\tau_{sj})}_{\ }ds}\ ,\\
\sqrt{\beta_{w}}\cos{(\Delta\phi_{wj})}\quad &\longrightarrow&\quad\label{eq:ICDwj}
J_{C_\Delta,wj}=\frac{1}{L_w}\int_0^{L_w}{\sqrt{\beta(s)}
                                          \cos{(\Delta\phi_{sj})}_{\ }ds}\ , \\
\sqrt{\beta_{w}}\beta_{m}\cos{(\tau_{wj})}\cos{(2\tau_{mw})}\ &\longrightarrow&\ 
   P_{C,mwj}=\frac{1}{L_mL_w}\label{eq:PC1}
   \int_0^{L_w}{\sqrt{\beta(s')}\cos{(\tau_{s'j})}
   \int_0^{L_m}{\beta(s'')\cos{(2\tau_{s''s'})}_{\ }ds''}\ ds'}\ ,\hskip1cm\\
\sqrt{\beta_{w}}\beta_{m}\sin{(\tau_{wj})}\sin{(2\tau_{mw})}\ &\longrightarrow&\ 
   P_{S,mwj}=\frac{1}{L_mL_w}\label{eq:PS1}
   \int_0^{L_w}{\sqrt{\beta(s')}\sin{(\tau_{s'j})}
   \int_0^{L_m}{\beta(s'')\sin{(2\tau_{s''s'})}_{\ }ds''}\ ds'}\ ,\\
\beta_{m}D_{m}\quad &\longrightarrow&\quad\label{eq:LBD}
L_{\beta D,m}=\frac{1}{L_m}\int_0^{L_m}{\beta(s)D(s)_{\ }ds}\ ,\\
\beta_{m,p}D_{m,q}\cos{(2\tau_{p,mj})}\quad &\longrightarrow&\quad\label{eq:LBDC}
L_{C_p,D_q,mj}=\frac{1}{L_m}\int_0^{L_m}{\beta_p(s)D_q(s)\cos{(2\tau_{p,sj})}_{\ }ds}\ ,
\qquad p,q=x,y\\
\beta_{m,p}D_{m,q}\sin{(2\tau_{p,mj})}\quad &\longrightarrow&\quad\label{eq:LBDS}
L_{S_p,D_q,mj}=\frac{1}{L_m}\int_0^{L_m}{\beta_p(s)D_q(s)\sin{(2\tau_{p,sj})}_{\ }ds}\ ,
\qquad p,q=x,y
\end{eqnarray}
where $L_w$ and $L_m$ denote the magnetic lengths,  
$s'$ and $s''$ represent the position inside the 
two magnets, and $\Delta\phi_{s}$ is the phase advance 
along either the steerer $w$ or the magnet $m$ ($\tau$ 
is the usual shifted phase advance).  

The same algebra carried out in the previous sections can 
be repeated by noting that an approximated transfer matrix 
for an orbit corrector or a sextupole reads
\begin{eqnarray}
\mathbf{A}(s)=\left(\begin{array}{c c}
1  & s \\ 0 & 1\end{array} \right) \quad  .\label{eq:AdefW}
\end{eqnarray}
This approximation is valid for sextupoles, as they do not 
alter the linear optics, whereas for steerers it holds 
for small deflection angles only. The few tens of 
$\mu$rad usually imparted during ORM measurements 
definitively meet this condition. From the same $C$ matrix 
of Eq.~\eqref{eq:Cdef1} the following relations hold
\begin{eqnarray}
\left\{\begin{aligned} A_{w,11}&=C_{w,11} \\ A_{w,12}&=C_{w,12}
       \end{aligned}\right. 
\Longrightarrow\left\{
\begin{aligned}
\sqrt{\beta(s)}\sin{\Delta\phi_s}&=\frac{s}{\sqrt{\beta_{w0}}} \\
\sqrt{\beta(s)}\cos{\Delta\phi_s}&=\sqrt{\beta_{w0}}
-\frac{\alpha_{w0}}{\sqrt{\beta_{w0}}}s
\end{aligned}\right. \quad ,\label{eq:CWmatrix}
\end{eqnarray}
where $\beta_{w0}$ and $\alpha_{w0}$ are the C-S parameters 
at the entrance of the steerer (as well as of the sextupole after 
replacing $w$ with $m$). The integrals across the 
magnet then reads
\begin{eqnarray}
\begin{aligned}
T_{S,w}&=\frac{1}{L_w}\int_0^{L_w}\frac{s}{\beta_{w0}}\ ds
       =\frac{L_w}{2\sqrt{\beta_{w0}}}\quad ,  \\
T_{C,w}&=\frac{1}{L_w}\int_0^{L_w}\left(\sqrt{\beta_{w0}}
              -\frac{\alpha_{w0}}{\beta_{w0}}s\right)\ ds
        =\sqrt{\beta_{w0}}-\frac{L_w}{2\sqrt{\beta_{w0}}}\quad .
\end{aligned}\label{eq:IWCS}
\end{eqnarray}
The integrals of Eqs.~\eqref{eq:ICwj}-\eqref{eq:ICDwj} can 
be then computed after noting that 
\begin{eqnarray}
\begin{aligned}
J_{S,wj}&=\sin{(\tau_{s_wj})}T_{C,w}-\cos{(\tau_{s_wj})}T_{S,w}\quad , \\
J_{C,wj}&=\cos{(\tau_{s_wj})}T_{C,w}+\sin{(\tau_{s_wj})}T_{S,w}\quad , \\
J_{C_\Delta,wj}&=\cos{(\Delta\phi_{s_wj})}T_{C,w}+\sin{(\Delta\phi_{s_wj})}
                 T_{S,w}\quad , \\
\end{aligned}\label{eq:IWCS2}
\end{eqnarray}
where $\Delta\phi_{s_wj}$ and $\tau_{s_{m}j}$ are the phase 
advance and the shifted phase advance, respectively, between 
the entrance of the steerer $w$ and the BPM $j$.

After some algebra the integrals $P_{C,mwj}$ and $P_{S,mwj}$ 
of Eqs.~\eqref{eq:PC1}-\eqref{eq:PS1} can be written as
\begin{eqnarray}
   P_{C,mwj}&=&\frac{1}{L_w}\nonumber %\label{eq:PC2}
   \int_0^{L_w}{\hskip-4mm\sqrt{\beta(s')}\Bigl[
      I_{C,mw_0}\cos{(2\Delta\phi_{s'})}
     -I_{S,mw_0}\sin{(2\Delta\phi_{s'})}\Bigr]\Bigl[
      \cos{(\tau_{w_0,j})}\cos{(\Delta\phi_{s'})}
     +\sin{(\tau_{w_0,j})}\sin{(\Delta\phi_{s'})}\Bigr]ds'}\ ,\\
   P_{S,mwj}&=&\frac{1}{L_w}\nonumber %\label{eq:PS2}
   \int_0^{L_w}{\hskip-4mm\sqrt{\beta(s')}\Bigl[
      I_{S,mw_0}\cos{(2\Delta\phi_{s'})}
     +I_{C,mw_0}\sin{(2\Delta\phi_{s'})}\Bigr]\Bigl[
      \sin{(\tau_{w_0,j})}\cos{(\Delta\phi_{s'})}
     -\cos{(\tau_{w_0,j})}\sin{(\Delta\phi_{s'})}\Bigr]ds'}\ ,
\end{eqnarray}
where $I_{C,mw_0}$ and  $I_{C,mw_0}$ are the same integrals 
across the magnet $m$ of Eq.~\eqref{eq:IS2}, with the location 
of the BPM $j$ replaced by $w_0$ which is the entrance of 
the steerer magnet $w$. It remains hence to integrate the 
trigonometric terms of $\Delta\phi_{s'}$, i.e. of the phase 
advance along the steerer $w$. To this end some approximations 
are necessary, by assuming that total phase advance the orbit 
corrector is sufficiently small ($\Delta\phi_w\ll 1$) so 
to have
\begin{eqnarray}
\cos{(2\Delta\phi_{s'})}\cos{(\Delta\phi_{s'})}\simeq&\nonumber
           1\hskip7mm +O(\Delta\phi_{s'}^2)\ &\simeq\cos{(\Delta\phi_{s'})}\ , \\
\sin{(2\Delta\phi_{s'})}\cos{(\Delta\phi_{s'})}\simeq&\ \nonumber
           2\Delta\phi_s+O(\Delta\phi_{s'}^3)\ &\simeq2\sin{(\Delta\phi_{s'})}\ , \\
\cos{(2\Delta\phi_{s'})}\sin{(\Delta\phi_{s'})}\simeq&\ \nonumber
           \ \Delta\phi_s+O(\Delta\phi_{s'}^2)\ &\simeq\sin{(\Delta\phi_{s'})}\ , \\
\sin{(2\Delta\phi_{s'})}\sin{(\Delta\phi_{s'})}\simeq&\nonumber
           0\hskip7mm +O(\Delta\phi_{s'}^2)\ &\simeq 0\ .
\end{eqnarray}
With these approximations the above integrals simplify to
\begin{eqnarray}
\begin{aligned}
   P_{C,mwj}&\simeq&\frac{1}{L_w}
   \int_0^{L_w}I_{C,mw_0}\Bigl[
      \cos{(\tau_{w_0,j})}\left(\sqrt{\beta(s')}\cos{(\Delta\phi_{s'})}\right)
     +\sin{(\tau_{w_0,j})}\left(\sqrt{\beta(s')}\sin{(\Delta\phi_{s'})}\right)
     \Bigr]- \\ && \hskip 12mm 2I_{S,mw_0}
      \cos{(\tau_{w_0,j})}\left(\sqrt{\beta(s')}\sin{(\Delta\phi_{s'})}\right)
     ds'  \\
   P_{S,mwj}&\simeq&\frac{1}{L_w}
   \int_0^{L_w}I_{S,mw_0}\Bigl[
      \sin{(\tau_{w_0,j})}\left(\sqrt{\beta(s')}\cos{(\Delta\phi_{s'})}\right)
     -\cos{(\tau_{w_0,j})}\left(\sqrt{\beta(s')}\sin{(\Delta\phi_{s'})}\right)
     \Bigr]+ \\ && \hskip 12mm 2I_{C,mw_0}
      \sin{(\tau_{w_0,j})}\left(\sqrt{\beta(s')}\sin{(\Delta\phi_{s'})}\right)
     ds'\ .
\end{aligned}\ . \label{eq:PC2}
\end{eqnarray}
The integrands in $s'$ within the large parenthesis are 
the same of Eq.~\eqref{eq:CWmatrix} and the above 
quantities read
\begin{eqnarray}
\begin{aligned}
   P_{C,mwj}&\simeq&
   I_{C,mw_0}\Bigl[\cos{(\tau_{w_0,j})}T_{C,w}
                  +\sin{(\tau_{w_0,j})}T_{S,w}\Bigr]
  -2I_{S,mw_0}T_{S,w}\cos{(\tau_{w_0,j})} \\
   P_{S,mwj}&\simeq&
   I_{S,mw_0}\Bigl[\sin{(\tau_{w_0,j})}T_{C,w}
                  -\cos{(\tau_{w_0,j})}T_{S,w}\Bigr]
  +2I_{C,mw_0}T_{S,w}\sin{(\tau_{w_0,j})}
\end{aligned}\ , \label{eq:PC3}
\end{eqnarray}
where $\tau_{w_0,j}$ is the same shifted phase advance between 
the entrance of the steerer $w$ and the BPM $j$ of 
Eq.~\eqref{eq:def_tau}, $T_{C,w}$ and $T_{S,w}$ are 
computed in Eq.~\eqref{eq:IWCS}, while $I_{C,mw_0}$ 
and $I_{S,mw_0}$ are to be evaluated via Eq.~\eqref{eq:IS2}.

Eq.~\eqref{eq:Nmatrix1} can be now rewritten in a more compact 
notation accounting for thick quadrupole magnets $m$ and orbit 
correctors $w$.
\begin{eqnarray}\nonumber 
N_{wj,m}&\simeq&\mp
  \frac{\sqrt{\beta_{j}^{(mod)}}}{2\sin{(\pi Q^{(mod)})}}
 \Bigg\{\frac{1}{4\sin{(2\pi Q^{(mod)})}}
              \Big[J_{C,wj}I_{C,mj}+P_{C,mwj}+J_{S,wj}I_{S,mj}-P_{S,mwj}\Big]
              \\ \nonumber &&\hspace{3.2cm}
        +\frac{1}{2}J_{S,wj}I_{\beta,m}\left[\Pi(m,j)-\Pi(m,w)+\Pi(j,w)\right]
       +\frac{J_{C_\Delta,wj}I_{\beta,m}}
            {4\sin{(\pi Q^{(mod)})}}\Bigg\}\ ,
\end{eqnarray}
where the sign is negative in the horizontal plane, positive in 
the vertical plane. $I_{\beta,m}$, $I_{C,mj}$ and $I_{S,mj}$ are 
the integrals across the quadrupoles of Eqs.~\eqref{eq:Ib2}-\eqref{eq:IS2}. 
$J_{C,wj}$, $J_{s,wj}$ and $J_{C_\Delta,wj}$ are the integrals across 
the steerer magnets of Eq.~\eqref{eq:IWCS2}, whereas the double 
integrals $P_{C,mwj}$ and $P_{S,mwj}$ are those of Eq.~\eqref{eq:PC3}.

The integral $L_{\beta D,m}$ can be used in the evaluation of linear 
chromaticity of Eq.~\eqref{eq:Text_Chrom1} when the 
variation of beta function and dispersion 
across a sextupole cannot be neglected. The magnet is here 
approximated as a drift. By summing up the square of the two 
equations in Eq.~\eqref{eq:CWmatrix} we obtain
\begin{eqnarray}\label{eq:beta}
\beta(s)=\beta_{m0}-2\alpha_{m0}s+\gamma_{m0}s^2 \quad,
\end{eqnarray}
whereas from Eqs.~\eqref{eq:Transport1} and~\eqref{eq:AdefW}
(for a drift $\vec{d}=(0 \ 0)^T$) the dispersion evolves linearly as 
\begin{eqnarray}\label{eq:Disp}
D(s)=D_{m0}+D'_{m0}s\quad .
\end{eqnarray}
The integral is then easily computed, resulting in 
\begin{eqnarray}
L_{\beta D,m}=\beta_{m0}D_{m0}
           +\left(\beta_{m0}D_{m0}'-2\alpha_{m0}D_{m0}\right)\frac{L_m}{2}
           +\left(\gamma_{m0}D_{m0}-2\alpha_{m0}D_{m0}'\right)\frac{L_m^2}{3}
           +\gamma_{m0}D_{m0}'\frac{L_m^3}{4}\quad . \label{eq:LBD2}
\end{eqnarray}

The integrals $L_{C_p,D_q,mj}$ and $L_{S_p,D_q,mj}$ (with $p$ 
and $q$ either $x$ or $y$) can be used in the evaluation of the 
chromatic beating of Eq.~\eqref{eq:Text_ChromBeat3} and 
of the chromatic phase advance shift of 
Eqs.~\eqref{eq:Text-ChromPhAdx}-\eqref{eq:Text-ChromPhAdy}, 
respectively. From Eqs.~\eqref{eq:CWmatrix},~\eqref{eq:beta} 
and~\eqref{eq:Disp} we can write
\begin{eqnarray}
\begin{aligned}
D_{q,m}(s)\beta_{p,m}(s)\cos{(2\Delta\phi_{p,s})}
     &=&D_{q,m}(s)\left[\beta_{p,m}(s)-2\beta_{p,m}(s)\sin{(\Delta\phi_{p,s})}^2\right]
        \hskip 3.8cm\\
     &=&\left(D_{m0,q}+D_{m0,q}'s\right)\left(\beta_{p,m0}-2\alpha_{p,m0}s
        +\gamma_{p,m0}s^2-\frac{2}{\beta_{p,m0}}s^2\right) 
     \hskip 0.6cm\quad ,\\
D_{q,m}(s)\beta_{p,m}(s)\sin{(2\Delta\phi_{p,s})}
     &=&2D_{q,m}(s)\left(\sqrt{\beta_{p,m}(s)}\sin{(\Delta\phi_{p,s})}\right)
        \left(\sqrt{\beta_{p,m}(s)}\cos{(\Delta\phi_{p,s})}\right)
     \hskip 1.2cm\\
     &=&2\left(D_{m0,q}+D_{m0,q}'s\right)\left(\frac{s}{\sqrt{\beta_{p,m0}}}\right)
        \left(\sqrt{\beta_{p,m0}}-\frac{\alpha_{p,m0}}{\sqrt{\beta_{p,m0}}}s\right)
     \hskip 1.2cm\quad .
\end{aligned}
\end{eqnarray}
The integrals along the magnetic length 
\begin{eqnarray}
\begin{aligned}
\mathcal{D}_{C_p,q,m}=\frac{1}{L_m}\int_0^{L_m}
        {D_{q,m}(s)\beta_{p,m}(s)\cos{(2\Delta\phi_{p,s})}_{\ }ds}\quad ,\\
\mathcal{D}_{S_p,q,m}=\frac{1}{L_m}\int_0^{L_m}
        {D_{q,m}(s)\beta_{p,m}(s)\sin{(2\Delta\phi_{p,s})}_{\ }ds}\quad ,
\end{aligned}
\end{eqnarray}
are then easily computed
\begin{eqnarray}
\begin{aligned}
\mathcal{D}_{C_p,q,m}&=D_{m0,q}\beta_{p,m0}
                     +\frac{L_m}{2}\left(D_{m0,q}'\beta_{p,m0}-2\alpha_{p,m0}D_{m0,q}\right)
                     +\frac{L_m^2}{3}\left(D_{m0,q}\frac{\alpha_{p,m0}^2-1}{\beta_{p,m0}}-2\alpha_{p,m0}D_{m0,q}'\right)
     \\ &\hskip 0.3cm+\frac{L_m^3}{4}\left(D_{m0,q}'\frac{\alpha_{p,m0}^2-1}{\beta_{p,m0}}\right)
             \quad ,\\
\mathcal{D}_{S_p,q,m}&=D_{m0,q}L_m
                     +\frac{2L_m^2}{3}\left(D_{m0,q}'-\frac{\alpha_{p,m0}}{\beta_{p,m0}}D_{m0,q}\right)
                     +\frac{L_m^3}{2}\left(D_{m0,q}'\frac{\alpha_{p,m0}}{\beta_{p,m0}}\right)
             \quad ,
\end{aligned}
\end{eqnarray}
The integrals of Eqs.~\eqref{eq:LBDC}-\eqref{eq:LBDS} can 
be then computed after noting that 
\begin{eqnarray}
\begin{aligned}
L_{S_p,D_q,mj}&=\sin{(2\tau_{s_mj})}\mathcal{D}_{C_p,q,m}
              -\cos{(2\tau_{s_mj})}\mathcal{D}_{S_p,q,m}\quad , \\
L_{C_p,D_q,mj}&=\cos{(2\tau_{s_mj})}\mathcal{D}_{C_p,q,m}
              +\sin{(2\tau_{s_mj})}\mathcal{D}_{S_p,q,m}\quad , \\
\end{aligned}\label{eq:LBDCS}
\end{eqnarray}
where, once again, $p$ and $q$ can be either 
$x$ or $y$.
